Fast multiplication of random dense matrices with fixed sparse matrices

This work focuses on accelerating the multiplication of a dense random matrix with a (fixed) sparse matrix, which is frequently used in sketching algorithms. We develop a novel scheme that takes advantage of blocking and recomputation (on-the-fly random number generation) to accelerate this operation. The techniques we propose decrease memory movement, thereby increasing the algorithm's parallel scalability in shared memory architectures. On the Intel Frontera architecture, our algorithm can achieve 2x speedups over libraries such as Eigen and Intel MKL on some examples. In addition, with 32 threads, we can obtain a parallel efficiency of up to approximately 45%. We also present a theoretical analysis for the memory movement lower bound of our algorithm, showing that under mild assumptions, it's possible to beat the data movement lower bound of general matrix-matrix multiply (GEMM) by a factor of $\sqrt M$, where $M$ is the cache size. Finally, we incorporate our sketching algorithm into a randomized least squares solver. For extremely over-determined sparse input matrices, we show that our results are competitive with SuiteSparse; in some cases, we obtain a speedup of 10x over SuiteSparse.

==> bibtex/bib/biblio.tex <==
@article{https://doi.org/10.48550/arxiv.2203.02798,
  doi = {10.48550/ARXIV.2203.02798},
  
  url = {https://arxiv.org/abs/2203.02798},
  
  author = {Sobczyk, Aleksandros and Gallopoulos, Efstratios},
  
  keywords = {Data Structures and Algorithms (cs.DS), Distributed, Parallel, and Cluster Computing (cs.DC), Mathematical Software (cs.MS), FOS: Computer and information sciences, FOS: Computer and information sciences, F.2.1; G.3; E.1, 65F50, 65F08, 65F20, 68W10, 68W20, 68P05},
  
  title = {pylspack: Parallel algorithms and data structures for sketching, column subset selection, regression and leverage scores},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International}
}

@inproceedings{matrix:signature,
author = {Kurt, S\"{u}reyya Emre and Sukumaran-Rajam, Aravind and Rastello, Fabrice and Sadayyapan, P.},
title = {Efficient Tiled Sparse Matrix Multiplication through Matrix Signatures},
year = {2020},
isbn = {9781728199986},
publisher = {IEEE Press},
abstract = {Tiling is a key technique to reduce data movement in matrix computations. While tiling is well understood and widely used for dense matrix/tensor computations, effective tiling of sparse matrix computations remains a challenging problem. This paper proposes a novel method to efficiently summarize the impact of the sparsity structure of a matrix on achievable data reuse as a one-dimensional signature, which is then used to build an analytical cost model for tile size optimization for sparse matrix computations. The proposed model-driven approach to sparse tiling is evaluated on two key sparse matrix kernels: Sparse Matrix - Dense Matrix Multiplication (SpMM) and Sampled Dense-Dense Matrix Multiplication (SDDMM). Experimental results demonstrate that model-based tiled SpMM and SDDMM achieve high performance relative to the current state-of-the-art.},
booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
articleno = {87},
numpages = {14},
keywords = {SpMM, sparse matrix signature, SpMDM, multi-core, sparse dense matrix multiplication, sparse tiling},
location = {Atlanta, Georgia},
series = {SC '20}
}

@article{roofline,
author = {Williams, Samuel and Waterman, Andrew and Patterson, David},
title = {Roofline: An Insightful Visual Performance Model for Multicore Architectures},
year = {2009},
issue_date = {April 2009},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {52},
number = {4},
issn = {0001-0782},
url = {https://doi.org/10.1145/1498765.1498785},
doi = {10.1145/1498765.1498785},
abstract = {The Roofline model offers insight on how to improve the performance of software and hardware.},
journal = {Commun. ACM},
month = {apr},
pages = {65–76},
numpages = {12}
}

@article{suitesparse,
author = {Davis, Timothy A. and Hu, Yifan},
title = {The University of Florida Sparse Matrix Collection},
year = {2011},
issue_date = {November 2011},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {38},
number = {1},
issn = {0098-3500},
url = {https://doi.org/10.1145/2049662.2049663},
doi = {10.1145/2049662.2049663},
abstract = {We describe the University of Florida Sparse Matrix Collection, a large and actively growing set of sparse matrices that arise in real applications. The Collection is widely used by the numerical linear algebra community for the development and performance evaluation of sparse matrix algorithms. It allows for robust and repeatable experiments: robust because performance results with artificially generated matrices can be misleading, and repeatable because matrices are curated and made publicly available in many formats. Its matrices cover a wide spectrum of domains, include those arising from problems with underlying 2D or 3D geometry (as structural engineering, computational fluid dynamics, model reduction, electromagnetics, semiconductor devices, thermodynamics, materials, acoustics, computer graphics/vision, robotics/kinematics, and other discretizations) and those that typically do not have such geometry (optimization, circuit simulation, economic and financial modeling, theoretical and quantum chemistry, chemical process simulation, mathematics and statistics, power networks, and other networks and graphs). We provide software for accessing and managing the Collection, from MATLAB™, Mathematica™, Fortran, and C, as well as an online search capability. Graph visualization of the matrices is provided, and a new multilevel coarsening scheme is proposed to facilitate this task.},
journal = {ACM Trans. Math. Softw.},
month = {dec},
articleno = {1},
numpages = {25},
keywords = {performance evaluation, multilevel algorithms, Graph drawing, sparse matrices}
}


@misc{murray2023randomized,
      title={Randomized Numerical Linear Algebra : A Perspective on the Field With an Eye to Software}, 
      author={Riley Murray and James Demmel and Michael W. Mahoney and N. Benjamin Erichson and Maksim Melnichenko and Osman Asif Malik and Laura Grigori and Piotr Luszczek and Michał Dereziński and Miles E. Lopes and Tianyu Liang and Hengrui Luo and Jack Dongarra},
      year={2023},
      eprint={2302.11474},
      archivePrefix={arXiv},
      primaryClass={math.NA},
      note={arXiv:2302.11474 v2}
}

@INPROCEEDINGS{nuclear,
  author={Aktulga, Hasan Metin and Buluç, Aydin and Williams, Samuel and Yang, Chao},
  booktitle={2014 IEEE 28th International Parallel and Distributed Processing Symposium}, 
  title={Optimizing Sparse Matrix-Multiple Vectors Multiplication for Nuclear Configuration Interaction Calculations}, 
  year={2014},
  volume={},
  number={},
  pages={1213-1222},
  doi={10.1109/IPDPS.2014.125}}


@INPROCEEDINGS{dynamical,
  author={Liu, Xing and Chow, Edmond and Vaidyanathan, Karthikeyan and Smelyanskiy, Mikhail},
  booktitle={2012 IEEE 26th International Parallel and Distributed Processing Symposium}, 
  title={Improving the Performance of Dynamical Simulations Via Multiple Right-Hand Sides}, 
  year={2012},
  volume={},
  number={},
  pages={36-47},
  doi={10.1109/IPDPS.2012.14}}


 @misc{intel, title={Inspector-executor sparse blas routines}, url={https://www.intel.com/content/www/us/en/docs/onemkl/developer-reference-c/2023-1/inspector-executor-sparse-blas-routines.html}, journal={Intel}, publisher={Developer Reference for Intel® oneAPI Math Kernel Library for C}} 

@inproceedings{CSB,
author = {Bulu\c{c}, Aydin and Fineman, Jeremy T. and Frigo, Matteo and Gilbert, John R. and Leiserson, Charles E.},
title = {Parallel Sparse Matrix-Vector and Matrix-Transpose-Vector Multiplication Using Compressed Sparse Blocks},
year = {2009},
isbn = {9781605586069},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1583991.1584053},
doi = {10.1145/1583991.1584053},
abstract = {This paper introduces a storage format for sparse matrices, called compressed sparse blocks (CSB), which allows both Ax and A,x to be computed efficiently in parallel, where A is an n\texttimes{}n sparse matrix with nnzen nonzeros and x is a dense n-vector. Our algorithms use Θ(nnz) work (serial running time) and Θ(√nlgn) span (critical-path length), yielding a parallelism of Θ(nnz/√nlgn), which is amply high for virtually any large matrix. The storage requirement for CSB is the same as that for the more-standard compressed-sparse-rows (CSR) format, for which computing Ax in parallel is easy but A,x is difficult. Benchmark results indicate that on one processor, the CSB algorithms for Ax and A,x run just as fast as the CSR algorithm for Ax, but the CSB algorithms also scale up linearly with processors until limited by off-chip memory bandwidth.},
booktitle = {Proceedings of the Twenty-First Annual Symposium on Parallelism in Algorithms and Architectures},
pages = {233–244},
numpages = {12},
keywords = {work, matrix transpose, parallelism, storage format, compressed sparse rows, matrix-vector multiplication, compressed sparse blocks, sparse matrix, compressed sparse columns, span, multithreaded algorithm},
location = {Calgary, AB, Canada},
series = {SPAA '09}
}



 @article{automatic_parallelization,
author = {Ravishankar, Mahesh and Eisenlohr, John and Pouchet, Louis-No\"{e}l and Ramanujam, J. and Rountev, Atanas and Sadayappan, P.},
title = {Automatic Parallelization of a Class of Irregular Loops for Distributed Memory Systems},
year = {2014},
issue_date = {September 2014},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {1},
number = {1},
issn = {2329-4949},
url = {https://doi.org/10.1145/2660251},
doi = {10.1145/2660251},
abstract = {Many scientific applications spend significant time within loops that are parallel, except for dependences from associative reduction operations. However these loops often contain data-dependent control-flow and array-access patterns. Traditional optimizations that rely on purely static analysis fail to generate parallel code in such cases.This article proposes an approach for automatic parallelization for distributed memory environments, using both static and runtime analysis. We formalize the computations that are targeted by this approach and develop algorithms to detect such computations. We also describe algorithms to generate a parallel inspector that performs a runtime analysis of control-flow and array-access patterns, and a parallel executor to take advantage of this information. The effectiveness of the approach is demonstrated on several benchmarks that were automatically transformed using a prototype compiler. For these, the inspector overheads and performance of the executor code were measured. The benefit on real-world applications was also demonstrated through similar manual transformations of an atmospheric modeling software.},
journal = {ACM Trans. Parallel Comput.},
month = {oct},
articleno = {7},
numpages = {37},
keywords = {Distributed-memory systems, inspector-executor, irregular applications, parallelization}
}

@inproceedings{optimizing_irregular_Shared,
author = {Min, Seung-Jai and Eigenmann, Rudolf},
title = {Optimizing Irregular Shared-Memory Applications for Clusters},
year = {2008},
isbn = {9781605581583},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1375527.1375566},
doi = {10.1145/1375527.1375566},
abstract = {Irregular applications pose challenges in optimizing communication, due to the difficulty of analyzing irregular data accesses accurately and efficiently. This challenge is especially big when translating irregular shared-memory applications to message-passing form for clusters. The lack of effective irregular data analysis in the translation system results in unnecessary or redundant communication, which limits application scalability. In this paper, we present a Lean Distributed Shared Memory (LDSM) system, which features a fast and accurate irregular data access (IDA) analysis. The analysis uses a region-based diff method and makes use of a runtime library that is optimized for irregular applications. We describe three optimizations that improve the LDSM system performance. A parallel array reduction transformation reduces overheads in the analysis. A packed communication optimization and a differential communication optimization effectively eliminate unnecessary and redundant messages. We evaluate the performance of the optimized LDSM system on a set of representative irregular benchmarks. The optimized LDSM executes irregular applications on average 45% faster than the hand-tuned MPI applications.},
booktitle = {Proceedings of the 22nd Annual International Conference on Supercomputing},
pages = {256–265},
numpages = {10},
keywords = {openMP, irregular data accesses, performance, runtime technique, MPI, compiler analysis},
location = {Island of Kos, Greece},
series = {ICS '08}
}


@inproceedings{10.1145/2737924.2738003,
author = {Venkat, Anand and Hall, Mary and Strout, Michelle},
title = {Loop and Data Transformations for Sparse Matrix Code},
year = {2015},
isbn = {9781450334686},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2737924.2738003},
doi = {10.1145/2737924.2738003},
abstract = {This paper introduces three new compiler transformations for representing and transforming sparse matrix computations and their data representations. In cooperation with run-time inspection, our compiler derives transformed matrix representations and associated transformed code to implement a variety of representations targeting different architecture platforms. This systematic approach to combining code and data transformations on sparse computations, which extends a polyhedral transformation and code generation framework, permits the compiler to compose these transformations with other transformations to generate code that is on average within 5% and often exceeds manually-tuned, high-performance sparse matrix libraries CUSP and OSKI. Additionally, the compiler-generated inspector codes are on average 1.5 faster than OSKI and perform comparably to CUSP, respectively.},
booktitle = {Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
pages = {521–532},
numpages = {12},
keywords = {loop transformations, sparse matrices, inspector/executor, polyhedral model, non-affine},
location = {Portland, OR, USA},
series = {PLDI '15}
}


@article{Loop_and_data,
author = {Venkat, Anand and Hall, Mary and Strout, Michelle},
title = {Loop and Data Transformations for Sparse Matrix Code},
year = {2015},
issue_date = {June 2015},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {50},
number = {6},
issn = {0362-1340},
url = {https://doi.org/10.1145/2813885.2738003},
doi = {10.1145/2813885.2738003},
abstract = {This paper introduces three new compiler transformations for representing and transforming sparse matrix computations and their data representations. In cooperation with run-time inspection, our compiler derives transformed matrix representations and associated transformed code to implement a variety of representations targeting different architecture platforms. This systematic approach to combining code and data transformations on sparse computations, which extends a polyhedral transformation and code generation framework, permits the compiler to compose these transformations with other transformations to generate code that is on average within 5% and often exceeds manually-tuned, high-performance sparse matrix libraries CUSP and OSKI. Additionally, the compiler-generated inspector codes are on average 1.5 faster than OSKI and perform comparably to CUSP, respectively.},
journal = {SIGPLAN Not.},
month = {jun},
pages = {521–532},
numpages = {12},
keywords = {loop transformations, inspector/executor, sparse matrices, polyhedral model, non-affine}
}

@inproceedings{liu,
author = {Liu, Xing and Smelyanskiy, Mikhail and Chow, Edmond and Dubey, Pradeep},
title = {Efficient Sparse Matrix-Vector Multiplication on X86-Based Many-Core Processors},
year = {2013},
isbn = {9781450321303},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2464996.2465013},
doi = {10.1145/2464996.2465013},
abstract = {Sparse matrix-vector multiplication (SpMV) is an important kernel in many scientific applications and is known to be memory bandwidth limited. On modern processors with wide SIMD and large numbers of cores, we identify and address several bottlenecks which may limit performance even before memory bandwidth: (a) low SIMD efficiency due to sparsity, (b) overhead due to irregular memory accesses, and (c) load-imbalance due to non-uniform matrix structures.We describe an efficient implementation of SpMV on the IntelR Xeon PhiTM Coprocessor, codenamed Knights Corner (KNC), that addresses the above challenges. Our implementation exploits the salient architectural features of KNC, such as large caches and hardware support for irregular memory accesses. By using a specialized data structure with careful load balancing, we attain performance on average close to 90% of KNC's achievable memory bandwidth on a diverse set of sparse matrices. Furthermore, we demonstrate that our implementation is 3.52x and 1.32x faster, respectively, than the best available implementations on dual IntelR XeonR Processor E5-2680 and the NVIDIA Tesla K20X architecture.},
booktitle = {Proceedings of the 27th International ACM Conference on International Conference on Supercomputing},
pages = {273–282},
numpages = {10},
keywords = {intel many integrated core architecture (intel mic), spmv, knights corner, intel xeon phi, esb format},
location = {Eugene, Oregon, USA},
series = {ICS '13}
}

@misc{bramas2018computing,
      title={Computing the sparse matrix vector product using block-based kernels without zero padding on processors with AVX-512 instructions}, 
      author={Berenger Bramas and Pavel Kus},
      year={2018},
      eprint={1801.01134},
      archivePrefix={arXiv},
      primaryClass={cs.DC}
}

@article{LSQR,
author = {Paige, Christopher C. and Saunders, Michael A.},
title = {LSQR: An Algorithm for Sparse Linear Equations and Sparse Least Squares},
year = {1982},
issue_date = {March 1982},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {8},
number = {1},
issn = {0098-3500},
url = {https://doi.org/10.1145/355984.355989},
doi = {10.1145/355984.355989},
journal = {ACM Trans. Math. Softw.},
month = {mar},
pages = {43–71},
numpages = {29}
}







@article{LSRN,
author = {Meng, Xiangrui and Saunders, Michael A. and Mahoney, Michael W.},
title = {LSRN: A Parallel Iterative Solver for Strongly Over- or Underdetermined Systems},
journal = {SIAM Journal on Scientific Computing},
volume = {36},
number = {2},
pages = {C95-C118},
year = {2014},
doi = {10.1137/120866580},

URL = { 
    
        https://doi.org/10.1137/120866580
    
    

},
eprint = { 
    
        https://doi.org/10.1137/120866580
    
    

}
,
    abstract = { We describe a parallel iterative least squares solver named \textttLSRN that is based on random normal projection. \textttLSRN computes the min-length solution to \$\min\_{x \in \mathbb{R}^n} \|A x - b\|\_2\$, where \$A \in \mathbb{R}^{m \times n}\$ with \$m \gg n\$ or \$m \ll n\$, and where \$A\$ may be rank-deficient. Tikhonov regularization may also be included. Since \$A\$ is involved only in matrix-matrix and matrix-vector multiplications, it can be a dense or sparse matrix or a linear operator, and LSRN automatically speeds up when \$A\$ is sparse or a fast linear operator. The preconditioning phase consists of a random normal projection, which is embarrassingly parallel, and a singular value decomposition of size \$\lceil \gamma \min(m,n) \rceil \times \min(m,n)\$, where \$\gamma\$ is moderately larger than \$1\$, e.g., \$\gamma = 2\$. We prove that the preconditioned system is well-conditioned, with a strong concentration result on the extreme singular values, and hence that the number of iterations is fully predictable when we apply LSQR or the Chebyshev semi-iterative method. As we demonstrate, the Chebyshev method is particularly efficient for solving large problems on clusters with high communication cost. Numerical results show that on a shared-memory machine, LSRN is very competitive with LAPACK's DGELSD and a fast randomized least squares solver called Blendenpik on large dense problems, and it outperforms the least squares solver from SuiteSparseQR on sparse problems without sparsity patterns that can be exploited to reduce fill-in. Further experiments show that LSRN scales well on an Amazon Elastic Compute Cloud cluster. }
}


@inproceedings{Random123,
author = {Salmon, John K. and Moraes, Mark A. and Dror, Ron O. and Shaw, David E.},
title = {Parallel Random Numbers: As Easy as 1, 2, 3},
year = {2011},
isbn = {9781450307710},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2063384.2063405},
doi = {10.1145/2063384.2063405},
abstract = {Most pseudorandom number generators (PRNGs) scale poorly to massively parallel high-performance computation because they are designed as sequentially dependent state transformations. We demonstrate that independent, keyed transformations of counters produce a large alternative class of PRNGs with excellent statistical properties (long period, no discernable structure or correlation). These counter-based PRNGs are ideally suited to modern multi-core CPUs, GPUs, clusters, and special-purpose hardware because they vectorize and parallelize well, and require little or no memory for state. We introduce several counter-based PRNGs: some based on cryptographic standards (AES, Threefish) and some completely new (Philox). All our PRNGs pass rigorous statistical tests (including TestU01's BigCrush) and produce at least 264 unique parallel streams of random numbers, each with period 2128 or more. In addition to essentially unlimited parallel scalability, our PRNGs offer excellent single-chip performance: Philox is faster than the CURAND library on a single NVIDIA GPU.},
booktitle = {Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis},
articleno = {16},
numpages = {12},
location = {Seattle, Washington},
series = {SC '11}
}

@article{xoshiro,
author = {Blackman, David and Vigna, Sebastiano},
title = {Scrambled Linear Pseudorandom Number Generators},
year = {2021},
issue_date = {December 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {47},
number = {4},
issn = {0098-3500},
url = {https://doi.org/10.1145/3460772},
doi = {10.1145/3460772},
abstract = {F2-linear pseudorandom number generators are very popular due to their high speed, to the ease with which generators with a sizable state space can be created, and to their provable theoretical properties. However, they suffer from linear artifacts that show as failures in linearity-related statistical tests such as the binary-rank and the linear-complexity test. In this article, we give two new contributions. First, we introduce two new F2-linear transformations that have been handcrafted to have good statistical properties and at the same time to be programmable very efficiently on superscalar processors, or even directly in hardware. Then, we describe some scramblers, that is, nonlinear functions applied to the state array that reduce or delete the linear artifacts, and propose combinations of linear transformations and scramblers that give extremely fast pseudorandom number generators of high quality. A novelty in our approach is that we use ideas from the theory of filtered linear-feedback shift registers to prove some properties of our scramblers, rather than relying purely on heuristics. In the end, we provide simple, extremely fast generators that use a few hundred bits of memory, have provable properties, and pass strong statistical tests.},
journal = {ACM Trans. Math. Softw.},
month = {sep},
articleno = {36},
numpages = {32},
keywords = {Pseudorandom number generators}
}


@article{sketching,
    author = {Ahfock, D C and Astle, W J and Richardson, S},
    title = "{Statistical properties of sketching algorithms}",
    journal = {Biometrika},
    volume = {108},
    number = {2},
    pages = {283-297},
    year = {2020},
    month = {07},
    abstract = "{Sketching is a probabilistic data compression technique that has been largely developed by the computer science community. Numerical operations on big datasets can be intolerably slow; sketching algorithms address this issue by generating a smaller surrogate dataset. Typically, inference proceeds on the compressed dataset. Sketching algorithms generally use random projections to compress the original dataset, and this stochastic generation process makes them amenable to statistical analysis. We argue that the sketched data can be modelled as a random sample, thus placing this family of data compression methods firmly within an inferential framework. In particular, we focus on the Gaussian, Hadamard and Clarkson–Woodruff sketches and their use in single-pass sketching algorithms for linear regression with huge samples. We explore the statistical properties of sketched regression algorithms and derive new distributional results for a large class of sketching estimators. A key result is a conditional central limit theorem for data-oblivious sketches. An important finding is that the best choice of sketching algorithm in terms of mean squared error is related to the signal-to-noise ratio in the source dataset. Finally, we demonstrate the theory and the limits of its applicability on two datasets.}",
    issn = {0006-3444},
    doi = {10.1093/biomet/asaa062},
    url = {https://doi.org/10.1093/biomet/asaa062},
    eprint = {https://academic.oup.com/biomet/article-pdf/108/2/283/37938896/asaa062.pdf},
}



@misc{bezanson2012julia,
      title={Julia: A Fast Dynamic Language for Technical Computing}, 
      author={Jeff Bezanson and Stefan Karpinski and Viral B. Shah and Alan Edelman},
      year={2012},
      eprint={1209.5145},
      archivePrefix={arXiv},
      primaryClass={cs.PL}
}

@misc{c++_xoshiro, title={Lemire/SIMDXORSHIFT: Fast random number generators: Vectorized (SIMD) version of xorshift128+}, url={https://github.com/lemire/SIMDxorshift}, journal={GitHub}, author={Lemire, Daniel and Frei, Oleksandr and Downs, Travis and TheIronBorn and Jones, Gareth}} 

@misc{loopvec, url={https://juliasimd.github.io/LoopVectorization.jl/latest/}, journal={Home · LoopVectorization.jl}} 

==> old/biblio.tex <==
@article{https://doi.org/10.48550/arxiv.2203.02798,
  doi = {10.48550/ARXIV.2203.02798},
  
  url = {https://arxiv.org/abs/2203.02798},
  
  author = {Sobczyk, Aleksandros and Gallopoulos, Efstratios},
  
  keywords = {Data Structures and Algorithms (cs.DS), Distributed, Parallel, and Cluster Computing (cs.DC), Mathematical Software (cs.MS), FOS: Computer and information sciences, FOS: Computer and information sciences, F.2.1; G.3; E.1, 65F50, 65F08, 65F20, 68W10, 68W20, 68P05},
  
  title = {pylspack: Parallel algorithms and data structures for sketching, column subset selection, regression and leverage scores},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International}
}

@inproceedings{matrix:signature,
author = {Kurt, S\"{u}reyya Emre and Sukumaran-Rajam, Aravind and Rastello, Fabrice and Sadayyapan, P.},
title = {Efficient Tiled Sparse Matrix Multiplication through Matrix Signatures},
year = {2020},
isbn = {9781728199986},
publisher = {IEEE Press},
abstract = {Tiling is a key technique to reduce data movement in matrix computations. While tiling is well understood and widely used for dense matrix/tensor computations, effective tiling of sparse matrix computations remains a challenging problem. This paper proposes a novel method to efficiently summarize the impact of the sparsity structure of a matrix on achievable data reuse as a one-dimensional signature, which is then used to build an analytical cost model for tile size optimization for sparse matrix computations. The proposed model-driven approach to sparse tiling is evaluated on two key sparse matrix kernels: Sparse Matrix - Dense Matrix Multiplication (SpMM) and Sampled Dense-Dense Matrix Multiplication (SDDMM). Experimental results demonstrate that model-based tiled SpMM and SDDMM achieve high performance relative to the current state-of-the-art.},
booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
articleno = {87},
numpages = {14},
keywords = {SpMM, sparse matrix signature, SpMDM, multi-core, sparse dense matrix multiplication, sparse tiling},
location = {Atlanta, Georgia},
series = {SC '20}
}

@article{roofline,
author = {Williams, Samuel and Waterman, Andrew and Patterson, David},
title = {Roofline: An Insightful Visual Performance Model for Multicore Architectures},
year = {2009},
issue_date = {April 2009},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {52},
number = {4},
issn = {0001-0782},
url = {https://doi.org/10.1145/1498765.1498785},
doi = {10.1145/1498765.1498785},
abstract = {The Roofline model offers insight on how to improve the performance of software and hardware.},
journal = {Commun. ACM},
month = {apr},
pages = {65–76},
numpages = {12}
}

@article{suitesparse,
author = {Davis, Timothy A. and Hu, Yifan},
title = {The University of Florida Sparse Matrix Collection},
year = {2011},
issue_date = {November 2011},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {38},
number = {1},
issn = {0098-3500},
url = {https://doi.org/10.1145/2049662.2049663},
doi = {10.1145/2049662.2049663},
abstract = {We describe the University of Florida Sparse Matrix Collection, a large and actively growing set of sparse matrices that arise in real applications. The Collection is widely used by the numerical linear algebra community for the development and performance evaluation of sparse matrix algorithms. It allows for robust and repeatable experiments: robust because performance results with artificially generated matrices can be misleading, and repeatable because matrices are curated and made publicly available in many formats. Its matrices cover a wide spectrum of domains, include those arising from problems with underlying 2D or 3D geometry (as structural engineering, computational fluid dynamics, model reduction, electromagnetics, semiconductor devices, thermodynamics, materials, acoustics, computer graphics/vision, robotics/kinematics, and other discretizations) and those that typically do not have such geometry (optimization, circuit simulation, economic and financial modeling, theoretical and quantum chemistry, chemical process simulation, mathematics and statistics, power networks, and other networks and graphs). We provide software for accessing and managing the Collection, from MATLAB™, Mathematica™, Fortran, and C, as well as an online search capability. Graph visualization of the matrices is provided, and a new multilevel coarsening scheme is proposed to facilitate this task.},
journal = {ACM Trans. Math. Softw.},
month = {dec},
articleno = {1},
numpages = {25},
keywords = {performance evaluation, multilevel algorithms, Graph drawing, sparse matrices}
}


@misc{murray2023randomized,
      title={Randomized Numerical Linear Algebra : A Perspective on the Field With an Eye to Software}, 
      author={Riley Murray and James Demmel and Michael W. Mahoney and N. Benjamin Erichson and Maksim Melnichenko and Osman Asif Malik and Laura Grigori and Piotr Luszczek and Michał Dereziński and Miles E. Lopes and Tianyu Liang and Hengrui Luo and Jack Dongarra},
      year={2023},
      eprint={2302.11474},
      archivePrefix={arXiv},
      primaryClass={math.NA},
      note={arXiv:2302.11474 v2}
}

@INPROCEEDINGS{nuclear,
  author={Aktulga, Hasan Metin and Buluç, Aydin and Williams, Samuel and Yang, Chao},
  booktitle={2014 IEEE 28th International Parallel and Distributed Processing Symposium}, 
  title={Optimizing Sparse Matrix-Multiple Vectors Multiplication for Nuclear Configuration Interaction Calculations}, 
  year={2014},
  volume={},
  number={},
  pages={1213-1222},
  doi={10.1109/IPDPS.2014.125}}


@INPROCEEDINGS{dynamical,
  author={Liu, Xing and Chow, Edmond and Vaidyanathan, Karthikeyan and Smelyanskiy, Mikhail},
  booktitle={2012 IEEE 26th International Parallel and Distributed Processing Symposium}, 
  title={Improving the Performance of Dynamical Simulations Via Multiple Right-Hand Sides}, 
  year={2012},
  volume={},
  number={},
  pages={36-47},
  doi={10.1109/IPDPS.2012.14}}


 @misc{intel, title={Inspector-executor sparse blas routines}, url={https://www.intel.com/content/www/us/en/docs/onemkl/developer-reference-c/2023-1/inspector-executor-sparse-blas-routines.html}, journal={Intel}, publisher={Developer Reference for Intel® oneAPI Math Kernel Library for C}} 

@inproceedings{CSB,
author = {Bulu\c{c}, Aydin and Fineman, Jeremy T. and Frigo, Matteo and Gilbert, John R. and Leiserson, Charles E.},
title = {Parallel Sparse Matrix-Vector and Matrix-Transpose-Vector Multiplication Using Compressed Sparse Blocks},
year = {2009},
isbn = {9781605586069},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1583991.1584053},
doi = {10.1145/1583991.1584053},
abstract = {This paper introduces a storage format for sparse matrices, called compressed sparse blocks (CSB), which allows both Ax and A,x to be computed efficiently in parallel, where A is an n\texttimes{}n sparse matrix with nnzen nonzeros and x is a dense n-vector. Our algorithms use Θ(nnz) work (serial running time) and Θ(√nlgn) span (critical-path length), yielding a parallelism of Θ(nnz/√nlgn), which is amply high for virtually any large matrix. The storage requirement for CSB is the same as that for the more-standard compressed-sparse-rows (CSR) format, for which computing Ax in parallel is easy but A,x is difficult. Benchmark results indicate that on one processor, the CSB algorithms for Ax and A,x run just as fast as the CSR algorithm for Ax, but the CSB algorithms also scale up linearly with processors until limited by off-chip memory bandwidth.},
booktitle = {Proceedings of the Twenty-First Annual Symposium on Parallelism in Algorithms and Architectures},
pages = {233–244},
numpages = {12},
keywords = {work, matrix transpose, parallelism, storage format, compressed sparse rows, matrix-vector multiplication, compressed sparse blocks, sparse matrix, compressed sparse columns, span, multithreaded algorithm},
location = {Calgary, AB, Canada},
series = {SPAA '09}
}



 @article{automatic_parallelization,
author = {Ravishankar, Mahesh and Eisenlohr, John and Pouchet, Louis-No\"{e}l and Ramanujam, J. and Rountev, Atanas and Sadayappan, P.},
title = {Automatic Parallelization of a Class of Irregular Loops for Distributed Memory Systems},
year = {2014},
issue_date = {September 2014},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {1},
number = {1},
issn = {2329-4949},
url = {https://doi.org/10.1145/2660251},
doi = {10.1145/2660251},
abstract = {Many scientific applications spend significant time within loops that are parallel, except for dependences from associative reduction operations. However these loops often contain data-dependent control-flow and array-access patterns. Traditional optimizations that rely on purely static analysis fail to generate parallel code in such cases.This article proposes an approach for automatic parallelization for distributed memory environments, using both static and runtime analysis. We formalize the computations that are targeted by this approach and develop algorithms to detect such computations. We also describe algorithms to generate a parallel inspector that performs a runtime analysis of control-flow and array-access patterns, and a parallel executor to take advantage of this information. The effectiveness of the approach is demonstrated on several benchmarks that were automatically transformed using a prototype compiler. For these, the inspector overheads and performance of the executor code were measured. The benefit on real-world applications was also demonstrated through similar manual transformations of an atmospheric modeling software.},
journal = {ACM Trans. Parallel Comput.},
month = {oct},
articleno = {7},
numpages = {37},
keywords = {Distributed-memory systems, inspector-executor, irregular applications, parallelization}
}

@inproceedings{optimizing_irregular_Shared,
author = {Min, Seung-Jai and Eigenmann, Rudolf},
title = {Optimizing Irregular Shared-Memory Applications for Clusters},
year = {2008},
isbn = {9781605581583},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1375527.1375566},
doi = {10.1145/1375527.1375566},
abstract = {Irregular applications pose challenges in optimizing communication, due to the difficulty of analyzing irregular data accesses accurately and efficiently. This challenge is especially big when translating irregular shared-memory applications to message-passing form for clusters. The lack of effective irregular data analysis in the translation system results in unnecessary or redundant communication, which limits application scalability. In this paper, we present a Lean Distributed Shared Memory (LDSM) system, which features a fast and accurate irregular data access (IDA) analysis. The analysis uses a region-based diff method and makes use of a runtime library that is optimized for irregular applications. We describe three optimizations that improve the LDSM system performance. A parallel array reduction transformation reduces overheads in the analysis. A packed communication optimization and a differential communication optimization effectively eliminate unnecessary and redundant messages. We evaluate the performance of the optimized LDSM system on a set of representative irregular benchmarks. The optimized LDSM executes irregular applications on average 45% faster than the hand-tuned MPI applications.},
booktitle = {Proceedings of the 22nd Annual International Conference on Supercomputing},
pages = {256–265},
numpages = {10},
keywords = {openMP, irregular data accesses, performance, runtime technique, MPI, compiler analysis},
location = {Island of Kos, Greece},
series = {ICS '08}
}


@inproceedings{10.1145/2737924.2738003,
author = {Venkat, Anand and Hall, Mary and Strout, Michelle},
title = {Loop and Data Transformations for Sparse Matrix Code},
year = {2015},
isbn = {9781450334686},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2737924.2738003},
doi = {10.1145/2737924.2738003},
abstract = {This paper introduces three new compiler transformations for representing and transforming sparse matrix computations and their data representations. In cooperation with run-time inspection, our compiler derives transformed matrix representations and associated transformed code to implement a variety of representations targeting different architecture platforms. This systematic approach to combining code and data transformations on sparse computations, which extends a polyhedral transformation and code generation framework, permits the compiler to compose these transformations with other transformations to generate code that is on average within 5% and often exceeds manually-tuned, high-performance sparse matrix libraries CUSP and OSKI. Additionally, the compiler-generated inspector codes are on average 1.5 faster than OSKI and perform comparably to CUSP, respectively.},
booktitle = {Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
pages = {521–532},
numpages = {12},
keywords = {loop transformations, sparse matrices, inspector/executor, polyhedral model, non-affine},
location = {Portland, OR, USA},
series = {PLDI '15}
}


@article{Loop_and_data,
author = {Venkat, Anand and Hall, Mary and Strout, Michelle},
title = {Loop and Data Transformations for Sparse Matrix Code},
year = {2015},
issue_date = {June 2015},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {50},
number = {6},
issn = {0362-1340},
url = {https://doi.org/10.1145/2813885.2738003},
doi = {10.1145/2813885.2738003},
abstract = {This paper introduces three new compiler transformations for representing and transforming sparse matrix computations and their data representations. In cooperation with run-time inspection, our compiler derives transformed matrix representations and associated transformed code to implement a variety of representations targeting different architecture platforms. This systematic approach to combining code and data transformations on sparse computations, which extends a polyhedral transformation and code generation framework, permits the compiler to compose these transformations with other transformations to generate code that is on average within 5% and often exceeds manually-tuned, high-performance sparse matrix libraries CUSP and OSKI. Additionally, the compiler-generated inspector codes are on average 1.5 faster than OSKI and perform comparably to CUSP, respectively.},
journal = {SIGPLAN Not.},
month = {jun},
pages = {521–532},
numpages = {12},
keywords = {loop transformations, inspector/executor, sparse matrices, polyhedral model, non-affine}
}

@inproceedings{liu,
author = {Liu, Xing and Smelyanskiy, Mikhail and Chow, Edmond and Dubey, Pradeep},
title = {Efficient Sparse Matrix-Vector Multiplication on X86-Based Many-Core Processors},
year = {2013},
isbn = {9781450321303},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2464996.2465013},
doi = {10.1145/2464996.2465013},
abstract = {Sparse matrix-vector multiplication (SpMV) is an important kernel in many scientific applications and is known to be memory bandwidth limited. On modern processors with wide SIMD and large numbers of cores, we identify and address several bottlenecks which may limit performance even before memory bandwidth: (a) low SIMD efficiency due to sparsity, (b) overhead due to irregular memory accesses, and (c) load-imbalance due to non-uniform matrix structures.We describe an efficient implementation of SpMV on the IntelR Xeon PhiTM Coprocessor, codenamed Knights Corner (KNC), that addresses the above challenges. Our implementation exploits the salient architectural features of KNC, such as large caches and hardware support for irregular memory accesses. By using a specialized data structure with careful load balancing, we attain performance on average close to 90% of KNC's achievable memory bandwidth on a diverse set of sparse matrices. Furthermore, we demonstrate that our implementation is 3.52x and 1.32x faster, respectively, than the best available implementations on dual IntelR XeonR Processor E5-2680 and the NVIDIA Tesla K20X architecture.},
booktitle = {Proceedings of the 27th International ACM Conference on International Conference on Supercomputing},
pages = {273–282},
numpages = {10},
keywords = {intel many integrated core architecture (intel mic), spmv, knights corner, intel xeon phi, esb format},
location = {Eugene, Oregon, USA},
series = {ICS '13}
}

@misc{bramas2018computing,
      title={Computing the sparse matrix vector product using block-based kernels without zero padding on processors with AVX-512 instructions}, 
      author={Berenger Bramas and Pavel Kus},
      year={2018},
      eprint={1801.01134},
      archivePrefix={arXiv},
      primaryClass={cs.DC}
}

@article{LSQR,
author = {Paige, Christopher C. and Saunders, Michael A.},
title = {LSQR: An Algorithm for Sparse Linear Equations and Sparse Least Squares},
year = {1982},
issue_date = {March 1982},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {8},
number = {1},
issn = {0098-3500},
url = {https://doi.org/10.1145/355984.355989},
doi = {10.1145/355984.355989},
journal = {ACM Trans. Math. Softw.},
month = {mar},
pages = {43–71},
numpages = {29}
}







@article{LSRN,
author = {Meng, Xiangrui and Saunders, Michael A. and Mahoney, Michael W.},
title = {LSRN: A Parallel Iterative Solver for Strongly Over- or Underdetermined Systems},
journal = {SIAM Journal on Scientific Computing},
volume = {36},
number = {2},
pages = {C95-C118},
year = {2014},
doi = {10.1137/120866580},

URL = { 
    
        https://doi.org/10.1137/120866580
    
    

},
eprint = { 
    
        https://doi.org/10.1137/120866580
    
    

}
,
    abstract = { We describe a parallel iterative least squares solver named \textttLSRN that is based on random normal projection. \textttLSRN computes the min-length solution to \$\min\_{x \in \mathbb{R}^n} \|A x - b\|\_2\$, where \$A \in \mathbb{R}^{m \times n}\$ with \$m \gg n\$ or \$m \ll n\$, and where \$A\$ may be rank-deficient. Tikhonov regularization may also be included. Since \$A\$ is involved only in matrix-matrix and matrix-vector multiplications, it can be a dense or sparse matrix or a linear operator, and LSRN automatically speeds up when \$A\$ is sparse or a fast linear operator. The preconditioning phase consists of a random normal projection, which is embarrassingly parallel, and a singular value decomposition of size \$\lceil \gamma \min(m,n) \rceil \times \min(m,n)\$, where \$\gamma\$ is moderately larger than \$1\$, e.g., \$\gamma = 2\$. We prove that the preconditioned system is well-conditioned, with a strong concentration result on the extreme singular values, and hence that the number of iterations is fully predictable when we apply LSQR or the Chebyshev semi-iterative method. As we demonstrate, the Chebyshev method is particularly efficient for solving large problems on clusters with high communication cost. Numerical results show that on a shared-memory machine, LSRN is very competitive with LAPACK's DGELSD and a fast randomized least squares solver called Blendenpik on large dense problems, and it outperforms the least squares solver from SuiteSparseQR on sparse problems without sparsity patterns that can be exploited to reduce fill-in. Further experiments show that LSRN scales well on an Amazon Elastic Compute Cloud cluster. }
}


@inproceedings{Random123,
author = {Salmon, John K. and Moraes, Mark A. and Dror, Ron O. and Shaw, David E.},
title = {Parallel Random Numbers: As Easy as 1, 2, 3},
year = {2011},
isbn = {9781450307710},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2063384.2063405},
doi = {10.1145/2063384.2063405},
abstract = {Most pseudorandom number generators (PRNGs) scale poorly to massively parallel high-performance computation because they are designed as sequentially dependent state transformations. We demonstrate that independent, keyed transformations of counters produce a large alternative class of PRNGs with excellent statistical properties (long period, no discernable structure or correlation). These counter-based PRNGs are ideally suited to modern multi-core CPUs, GPUs, clusters, and special-purpose hardware because they vectorize and parallelize well, and require little or no memory for state. We introduce several counter-based PRNGs: some based on cryptographic standards (AES, Threefish) and some completely new (Philox). All our PRNGs pass rigorous statistical tests (including TestU01's BigCrush) and produce at least 264 unique parallel streams of random numbers, each with period 2128 or more. In addition to essentially unlimited parallel scalability, our PRNGs offer excellent single-chip performance: Philox is faster than the CURAND library on a single NVIDIA GPU.},
booktitle = {Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis},
articleno = {16},
numpages = {12},
location = {Seattle, Washington},
series = {SC '11}
}

@article{xoshiro,
author = {Blackman, David and Vigna, Sebastiano},
title = {Scrambled Linear Pseudorandom Number Generators},
year = {2021},
issue_date = {December 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {47},
number = {4},
issn = {0098-3500},
url = {https://doi.org/10.1145/3460772},
doi = {10.1145/3460772},
abstract = {F2-linear pseudorandom number generators are very popular due to their high speed, to the ease with which generators with a sizable state space can be created, and to their provable theoretical properties. However, they suffer from linear artifacts that show as failures in linearity-related statistical tests such as the binary-rank and the linear-complexity test. In this article, we give two new contributions. First, we introduce two new F2-linear transformations that have been handcrafted to have good statistical properties and at the same time to be programmable very efficiently on superscalar processors, or even directly in hardware. Then, we describe some scramblers, that is, nonlinear functions applied to the state array that reduce or delete the linear artifacts, and propose combinations of linear transformations and scramblers that give extremely fast pseudorandom number generators of high quality. A novelty in our approach is that we use ideas from the theory of filtered linear-feedback shift registers to prove some properties of our scramblers, rather than relying purely on heuristics. In the end, we provide simple, extremely fast generators that use a few hundred bits of memory, have provable properties, and pass strong statistical tests.},
journal = {ACM Trans. Math. Softw.},
month = {sep},
articleno = {36},
numpages = {32},
keywords = {Pseudorandom number generators}
}


@article{sketching,
    author = {Ahfock, D C and Astle, W J and Richardson, S},
    title = "{Statistical properties of sketching algorithms}",
    journal = {Biometrika},
    volume = {108},
    number = {2},
    pages = {283-297},
    year = {2020},
    month = {07},
    abstract = "{Sketching is a probabilistic data compression technique that has been largely developed by the computer science community. Numerical operations on big datasets can be intolerably slow; sketching algorithms address this issue by generating a smaller surrogate dataset. Typically, inference proceeds on the compressed dataset. Sketching algorithms generally use random projections to compress the original dataset, and this stochastic generation process makes them amenable to statistical analysis. We argue that the sketched data can be modelled as a random sample, thus placing this family of data compression methods firmly within an inferential framework. In particular, we focus on the Gaussian, Hadamard and Clarkson–Woodruff sketches and their use in single-pass sketching algorithms for linear regression with huge samples. We explore the statistical properties of sketched regression algorithms and derive new distributional results for a large class of sketching estimators. A key result is a conditional central limit theorem for data-oblivious sketches. An important finding is that the best choice of sketching algorithm in terms of mean squared error is related to the signal-to-noise ratio in the source dataset. Finally, we demonstrate the theory and the limits of its applicability on two datasets.}",
    issn = {0006-3444},
    doi = {10.1093/biomet/asaa062},
    url = {https://doi.org/10.1093/biomet/asaa062},
    eprint = {https://academic.oup.com/biomet/article-pdf/108/2/283/37938896/asaa062.pdf},
}



@misc{bezanson2012julia,
      title={Julia: A Fast Dynamic Language for Technical Computing}, 
      author={Jeff Bezanson and Stefan Karpinski and Viral B. Shah and Alan Edelman},
      year={2012},
      eprint={1209.5145},
      archivePrefix={arXiv},
      primaryClass={cs.PL}
}

@misc{c++_xoshiro, title={Lemire/SIMDXORSHIFT: Fast random number generators: Vectorized (SIMD) version of xorshift128+}, url={https://github.com/lemire/SIMDxorshift}, journal={GitHub}, author={Lemire, Daniel and Frei, Oleksandr and Downs, Travis and TheIronBorn and Jones, Gareth}} 

@misc{loopvec, url={https://juliasimd.github.io/LoopVectorization.jl/latest/}, journal={Home · LoopVectorization.jl}} 
